Aux-Drop: Handling Haphazard Inputs in Online Learning Using Auxiliary Dropouts

Many real-world applications based on online learning produce streaming data that is haphazard in nature, i.e., contains missing features, features becoming obsolete in time, the appearance of new features at later points in time and a lack of clarity on the total number of input features. These challenges make it hard to build a learnable system for such applications, and almost no work exists in deep learning that addresses this issue. In this paper, we present Aux-Drop, an auxiliary dropout regularization strategy for online learning that handles the haphazard input features in an effective manner. Aux-Drop adapts the conventional dropout regularization scheme for the haphazard input feature space ensuring that the final output is minimally impacted by the chaotic appearance of such features. It helps to prevent the co-adaptation of especially the auxiliary and base features, as well as reduces the strong dependence of the output on any of the auxiliary inputs of the model. This helps in better learning for scenarios where certain features disappear in time or when new features are to be modelled. The efficacy of Aux-Drop has been demonstrated through extensive numerical experiments on SOTA benchmarking datasets that include Italy Power Demand, HIGGS, SUSY and multiple UCI datasets. The code is available at https://github.com/Rohit102497/Aux-Drop.

==> ImageTex/ObsoleteAndSuddenResult.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=\textwidth, trim={4.0cm 18.2cm 1.2cm 5.3cm}, clip]{Images/ObsoleteAndSuddenResult.pdf} 
    \end{center}
    \caption{Result of the obsolete and sudden features experiment on (a) SUSY and (b) HIGGS dataset. We calculate the average number of errors in each 50k instances. Thus, the graph starts at 50k and goes till 1000k. B. F. \{n\} and A. F. \{n\} represents the $n\textsuperscript{th}$ number base features and auxiliary feature, respectively. The green box represents the time instances when a certain auxiliary feature was available. The x-axis denotes the number of instances (in k).}
    \label{fig:ObsoleteAndSuddenResult}
\end{figure*}

==> ImageTex/VariablePHIGGSandSUSYdiagram.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=\textwidth]{Images/VariableP_HIGGSandSUSY.png} 
    \end{center}
    \caption{Result}
    \label{fig:ObsoleteAndSuddenResult}
\end{figure*}

==> Tables/ComparisonWithOLVF.tex <==
\begin{table}
  \caption{Comparison with OLVF on various datasets. Here all the errors reported for OLVF is on 25\% of the data. Thus, we adjust the probability value for haphazard features for Aux-Drop accordingly to match the amount of missingness of OLVF. The error is reported as mean $\pm$ standard deviation of the 20 experiments performed randomly.}
  \vskip 0.15in
  \label{TabCompareOLVF25per}
  \centering
  \begin{tabular}{lccc}
  \hline
  \textbf{Dataset} & \textbf{OLVF} & \textbf{Aux-Drop} & \textbf{p} \\
  \hline
  german & 333.4 $\pm$ 9.7 & \textbf{317.4 $\pm$ 1.9} & .27\\
  svmguide3 & 346.4 $\pm$ 11.6 & \textbf{296.9 $\pm$ 1.5} & .28\\
  magic04 & 6152.4 $\pm$ 54.7 & \textbf{6039.1 $\pm$ 190.4} & .32\\
  a8a & 8993.8 $\pm$ 40.3 & \textbf{7855.5 $\pm$ 16.8} & .25\\
  \hline
  \end{tabular}
 \end{table}

==> Tables/IMDBdataset.tex <==
\begin{table}
  \caption{Experiment on IMDB dataset. The metric for comparison with OLVF and OCDS is mean $\pm$ standard deviation of the number of errors and the average accuracy respectively.}
  \vskip 0.15in
  \label{TabIMDBdataset}
  \centering
  \begin{tabular}{cc|c|c}
  \hline
  % \multirow{2}\textbf{OLSF} & \multirow{2}\textbf{OLVF} & \textbf{Aux-Drop} \\
  \multirow{2}{*}{\textbf{OLSF}} & \multirow{2}{*}{\textbf{OLVF}} & \multicolumn{2}{c}{\textbf{Aux-Drop}} \\ \cline{3-4}
  & & train & test \\
  \hline
  7851.0$\pm$51.4 & 4474.2 $\pm$ 39.1 & \\ 
  \hline
  \end{tabular}
 \end{table}

==> Tables/IPDD_Pvar_Aux12.tex <==
 \begin{table}
\floatbox[\capbeside]{table}
{\caption{The table contains the average loss on the Italy Power Demand dataset. The first 12 features are base features and the last 12 features are auxiliary features. The availability of each auxiliary feature is varied by a uniform distribution of probability $p$. The value of $p$ ranges from .50 to .99. The average loss of Aux-Net for each $p$ is reported from the Aux-Net paper \citep{agarwal2020auxiliary}. Aux-Drop is run five times and the mean of the average loss is reported here. }\label{TabMainIPDDPvarAux12}}%
{\begin{tabular}{lcc}
\hline
  \textbf{Probability} & \textbf{Aux-Net} & \textbf{Aux-Drop)} \\
  \hline
  .50 & .6975 & \textbf{.6118}\\
  .60 & .6831 & \textbf{.5722}\\
  .70 & .6788 & \textbf{.6099}\\
  .80 & .6130 & \textbf{.5613}\\
  .90 & .5456 & \textbf{.5355}\\
  .95 & .5168 & \textbf{.4971}\\
  .99 & .5165 & \textbf{.5001}\\
  \hline
\end{tabular}}
\vspace{-2mm}
\end{table}

==> Tables/PositionOfAuxLayer.tex <==
\begin{table}
  \caption{Comparison of the position of AuxLayer. Pos here stands for the position. The experiment is conducted on the four UCI datasets. The total number of hidden layers in the ODL is 6 for this experiment.}
  \label{TabPosOfAuxLayer}
  \centering
  \begin{tabular}{lcccc}
  \hline
  Pos & german & svmguide3 & magic04 & a8a \\
  \hline
  2 & 319.1$\pm$3.5 & 298.4$\pm$2.8 & 6054.0$\pm$213.3 & \textbf{7730.5$\pm$73.5}\\
  3 & \textbf{317.4$\pm$1.9} & \textbf{296.9$\pm$1.5} & \textbf{6039.1$\pm$190.4} & 7855.4$\pm$16.8\\
  4 & 318.5$\pm$2.7 & 298.9$\pm$2.8 & 6110.7$\pm$146.2 & 7852.9$\pm$12.4\\
  5 & 317.7$\pm$2.2 & 297.4$\pm$1.7 & 6428.7$\pm$105.5 & 7856.7$\pm$14.3\\
  \hline
  \end{tabular}
 \end{table}

==> Tables/Table4.tex <==
\begin{table}[]
  \centering
   \caption{Comparison with OLVF on various datasets. Here all the errors reported for OLVF are on 25\% of the data and the value is taken from its original paper. Thus, we adjust the probability value (p) for haphazard features for Aux-Drop accordingly to match the amount of missingness of OLVF. The error is reported as the mean $\pm$ standard deviation of the 20 experiments performed with random seeds.}
  \begin{tabular}{l|cccc}
  \hline
  \textbf{Dataset} & \textbf{OLVF} & \textbf{Aux-Drop(ODL)} & \textbf{Aux-Drop(OGD)} & \textbf{p} \\
  \hline
  german & 333.4$\pm$9.7 & \textbf{317.4$\pm$1.9} & 319.3$\pm$3.3 & .27\\
  svmguide3 & 346.4$\pm$11.6 & \textbf{296.9$\pm$1.5} & 297.5$\pm$1.2 & .28\\
  magic04 & 6152.4$\pm$54.7 & 6039.1$\pm$190.4 & \textbf{5796.0$\pm$219.1} & .32\\
  a8a & 8993.8$\pm$40.3 & 7855.5$\pm$16.8 & \textbf{7846.3$\pm$8.7} & .25\\
  \hline
  \end{tabular}
  \label{TabCompareOLVF25per}
\end{table}



==> Tables/Table4_5.tex <==
\begin{minipage}[b]{.45\textwidth}
  \centering
   \captionof{table}{Comparison with OLVF on various datasets. Here all the errors reported for OLVF are on 25\% of the data. Thus, we adjust the probability value (p) for haphazard features for Aux-Drop accordingly to match the amount of missingness of OLVF. The error is reported as the mean $\pm$ standard deviation of the 20 experiments performed randomly.}
  \begin{tabular}{l|ccc}
  \hline
  \textbf{Dataset} & \textbf{OLVF} & \textbf{Aux-Drop(ODL)} & \textbf{p} \\
  \hline
  german & 333.4$\pm$9.7 & \textbf{317.4$\pm$1.9} & .27\\
  svmguide3 & 346.4$\pm$11.6 & \textbf{296.9$\pm$1.5} & .28\\
  magic04 & 6152.4$\pm$54.7 & \textbf{6039.1$\pm$190.4} & .32\\
  a8a & 8993.8$\pm$40.3 & \textbf{7855.5$\pm$16.8} & .25\\
  \hline
  \end{tabular}
  \label{TabCompareOLVF25per}
\end{minipage}
\hspace{10mm}
\begin{minipage}[b]{.45\textwidth}
  \centering
  \captionof{table}{Experiments on the Trapezoidal data streams. The dataset for each row is similar to dataset of Table \ref{TabCompareOLVF25per}. Aux-Drop is compared with OLSF and OLVF (metrics reported from their original paper) in terms of the average number of errors.  All the experiments are performed 20 times and the mean $\pm$ standard deviation is reported.}
  \begin{tabular}{ccc}
  \hline
  \textbf{OLSF} & \textbf{OLVF} & \textbf{Aux-Drop(ODL)} \\
  \hline
  385.5$\pm$10.2 & 329.2$\pm$9.8 & \textbf{312.2$\pm$8.0}\\
  361.7$\pm$29.7 & 351.6$\pm$25.9 & \textbf{296.9$\pm$1.0} \\
  6147.4$\pm$65.3 & \textbf{5784.0$\pm$52.7} & 6361.25$\pm$319.6\\
  9420.4$\pm$549.9 & 8649.8$\pm$526.7 & \textbf{7855.4$\pm$16.8}\\
  \hline
  \end{tabular}
  \label{TabTrapezoidalStream}
\end{minipage}
  

==> Tables/TrapezoidalStreams.tex <==
\begin{table}
  \caption{Experiments on the Trapezoidal data streams. Aux-Drop is compared with OLSF and OLVF in terms of the average number of errors made.}
  \vskip 0.15in
  \label{TabTrapezoidalStream}
  \centering
  % \begin{adjustbox}{width=\columnwidth}
  \begin{tabular}{lccc}
  \hline
  \textbf{Dataset} & \textbf{OLSF} & \textbf{OLVF} & \textbf{Aux-Drop} \\
  \hline
  german & 385.5$\pm$10.2 & 329.2$\pm$9.8 & \textbf{312.2$\pm$8.0}\\
  svmguide3 & 361.7$\pm$29.7 & 351.6$\pm$25.9 & \textbf{296.9$\pm$1.0} \\
  magic04 & 6147.4$\pm$65.3 & \textbf{5784.0$\pm$52.7} & 6361.25$\pm$319.6\\
  a8a & 9420.4$\pm$549.9 & 8649.8$\pm$526.7 & \textbf{7855.4$\pm$16.8}\\
  \hline
  \end{tabular}
 \end{table}

==> Tables/variablePHIGGSandSUSY.tex <==
\begin{table}\centering
\caption{Error in HIGGS and SUSY for various probability $p$. The metric is reported as the mean $\pm$ standard deviation of the number of errors in 5 runs. The error of ODL trained on only base features for HIGGS dataset is 441483.2$\pm$184.3. The error of ODL(B) for SUSY dataset is 286198.6$\pm$189.4.  The value reported in the table is calculated by subtracting the average number of errors and standard deviation of ODL(B) with the average number of errors and standard deviation of Aux-Drop, respectively.}
\label{TabVariablePHiggsAndSUSYbaseODL}
\vskip 0.15in

\begin{tabular}{|c|c|c|}
\hline
$p$$ & HIGGS & SUSY \\
\hline
  .01 & 1500$\pm$(-54.4) & 1111$\pm$(-120.1)\\
  .05  & 1438$\pm$(+66.2) & 2736$\pm$(+116.1)\\
  .1  & 1731$\pm$(+14.2) & 5446$\pm$(+206.8)\\
  .2  & 2708$\pm$(+177.4) & 11292$\pm$(+386.3)\\
  .3  & 6197$\pm$(+491.2) & 16929$\pm$(+360.2)\\
  .4  & 9292$\pm$(+197) & 23485$\pm$(+442.9)\\
  .5  & 13638$\pm$(+431.8) & 29479$\pm$(+428.9)\\
  .6 & 18480$\pm$(+420.1) & 36091$\pm$(+640.1)\\
  .7 & 22556$\pm$(+310.9) & 42244$\pm$(+624.3)\\
  .8 & 28882$\pm$(+69.7) & 48987$\pm$(+465.1)\\
  .9 & 35649$\pm$(+166) & 55982$\pm$(+509.1)\\
  .95 & 42248$\pm$(+429.4) & 59567$\pm$(+165.0)\\
  .99 & 49695$\pm$(+457.5) & 64047$\pm$(-8.0)\\
\hline
\end{tabular}
  
\end{table}




